Confident Sinkhorn Allocation for Pseudo-Labeling

Semi-supervised learning is a critical tool in reducing machine learning's dependence on labeled data. It has been successfully applied to structured data, such as images and natural language, by exploiting the inherent spatial and semantic structure therein with pretrained models or data augmentation. These methods are not applicable, however, when the data does not have the appropriate structure, or invariances. Due to their simplicity, pseudo-labeling (PL) methods can be widely used without any domain assumptions. However, the greedy mechanism in PL is sensitive to a threshold and can perform poorly if wrong assignments are made due to overconfidence. This paper studies theoretically the role of uncertainty to pseudo-labeling and proposes Confident Sinkhorn Allocation (CSA), which identifies the best pseudo-label allocation via optimal transport to only samples with high confidence scores. CSA outperforms the current state-of-the-art in this practically important area of semi-supervised learning. Additionally, we propose to use the Integral Probability Metrics to extend and improve the existing PACBayes bound which relies on the Kullback-Leibler (KL) divergence, for ensemble models. Our code is publicly available at https://github.com/amzn/confident-sinkhorn-allocation.

==> 2.related_work.tex <==




% $\pi$-Model: The simplest setting in which to apply consistency regularization is when the prediction function $f_\theta(x)$ is itself stochastic, i.e. it can produce different outputs for the same input x.
% This is quite common in practice during training when $f_\theta(x)$ is a neural network due to common
% regularization techniques such as data augmentation, dropout, and adding noise. $\pi$-Model \cite{sajjadi2016regularization,zheng2021rectifying} 
% adds a loss term which encourages the distance between a network's output for different passes of
% $x \in DUL$ through the network to be small.


% Mean Teacher: A difficulty with the $\pi$-model approach is that it relies on a potentially unstable
% target prediction, namely the second stochastic network prediction which can rapidly change over
% the course of training. As a result, \cite{tarvainen2017mean} proposed to obtain a more stable target output $f_\theta(x)$ for
% $x \in DUL$ by setting the target to predictions made using an exponential moving average of parameters
% from previous training steps.


%Virtual Adversarial Training: Instead of relying on the built-in stochasticity of $f_\theta(x)$, Virtual Adversarial Training (VAT) [39] directly approximates a tiny perturbation radv to add to x which would most significantly affect the output of the prediction function.

%Existing work in SSL includes Entropy Minimization \cite{grandvalet2004semi} which adds a loss term applied that encourages the network to make confident (low-entropy) predictions for all unlabeled examples, regardless of their class. 

%There are a wide class of SSL methods including $\pi$-Model \cite{sajjadi2016regularization,zheng2021rectifying}, Mean Teacher \cite{tarvainen2017mean}, MixMatch \cite{berthelot2019mixmatch}, FixMatch \cite{sohn2020fixmatch}, FlexMatch \cite{zhang2021flexmatch}. However, such approaches may not be applicable for tabular data where neither data augmentation nor pretraining is available. 

%We briefly review a few methods applicable for tabular setting considered in this paper.

% assigns fake labels to unlabeled samples based on the maximum probabilities predicted by the current model and then trains the model on both labeled and unlabeled samples simultaneously in a pure supervised setup.


% Why could pseudo labels work? Pseudo label is in effect equivalent to Entropy Regularization (Grandvalet & Bengio 2004), which minimizes the conditional entropy of class probabilities for unlabeled data to favor low density separation between classes. In other words, the predicted class probabilities is in fact a measure of class overlap, minimizing the entropy is equivalent to reduced class overlap and thus low density separation.



%While we previously argue that existing data augmentation methods for SSL are not applicable to tabular data setting where the structured images, text or pretrained models are not available.
\textbf{Consistency assumption for tabular data.} Despite the challenges, Yoon~\emph{et al.}~\cite{yoon2020vime} perform data augmentation for tabular data by estimating mask vectors from corrupted tabular data in addition to the reconstruction pretext task. Their method (Vime) uses an encoder function to learn the representation from tabular data and generate multiple augmented samples for each data point by hallucination using several
different masks then imputing the corrupted values for each masked data point. Another work \cite{darabi2021contrastive} proposes a mixup-based augmentation under the manifold assumption by mapping samples to a low dimensional latent space and encouraging interpolated samples to have high similarity within the same labeled class. %Unlabeled samples are additionally employed via a transductive label propagation method to further enrich the set of similar and dissimilar pairs that can be used in the contrastive loss term.
However, one of the key drawback is that the deep learning components of both approaches need access to \textit{large amounts}\footnote{The dataset sizes range from 48k (Adult) to 2.9M (UK Biobank) \cite{yoon2020vime}} of unlabelled data so that the constrastive learning and data augmentation can be learned effectively. %In particular, the datasets range from 48k (adult) to 2.9M (UKBiobank) wherein they consider the number of labelled samples is $10\%$ and the remaining $90\%$ samples as unlabeled set.

%The goal of pseudo-labeling \cite{lee2013pseudo} and self-training \cite{yarowsky1995unsupervised} is to generate pseudo-labels for unlabeled samples with a model trained on labeled data. In \cite{lee2013pseudo}, pseudo-labels are created from the predictions of a trained neural network. Pseudo-labels can also be assigned to unlabeled samples based on neighborhood graphs \cite{iscen2019label}. \cite{shi2018transductive} extend the idea of pseudo-labeling by incorporating confidence scores for unlabeled samples based on the density of a local neighborhood. There are other works \cite{wang2020repetitive,xie2020self,haase2021iterative} trying to improve the performance of deep learning via self-training.


%Although previous pseudo-labeling based SSL approaches are general and domain-agnostic, they tend to under-perform due to the generation of noisy pseudo-labels; our approach greatly reduces noise by minimizing the effect of poor network calibration, allowing for competitive state-of-the-art results.


%This happens, for example, when we have limited number of samples (including labeled and unlabeled). Thus, we can not use deep network to learn the latent embedding representation for generating the augmentation. 




\textbf{When consistency assumption is not available.} We can use pseudo-labeling (PL) \cite{lee2013pseudo} to generate `pseudo-labels' for unlabeled samples with a model trained on labeled data. A label $k$ is assigned to an unlabelled sample $\bx_i$ where a predicted class probability is larger than a predefined threshold $\gamma$ as %Using the predictive probabilities, the pseudo-label can be generated for a data point $\bx_i$ as: 
\begin{align}
    y_i^k = \mathbb{1} \Bigl[ p( y_i = k \mid \bx_i ) \ge \gamma \Bigr]
\end{align}
where $\gamma \in (0,1)$ is a threshold used to produce hard labels and $p( y_i = k \mid \bx_i )$ is the predictive probability of the $i$-th data point  belonging to the class $k$-th.  
%A Then, the classifier is trained using both labeled and unlabeled samples simultaneously in a purely supervised setup.  
A classifier can then be trained using both the original labelled data and the newly pseudo-labelled data.
Pseudo labeling is naturally an iterative process, with the next round of pseudo-labels being generated using the most-recently trained classifier.  The key advantage of pseudo-labeling  is that it does not inherently require augmentations and can be generally applied to most domains, including tabular data. 
%over consistency regularization Due to its simplicity, PL can be widely applicable for tabular domains.

 While the standard pseudo-labeling method relies on a predefined single threshold $\gamma$ for all classes, FlexMatch \cite{zhang2021flexmatch} has extended this mechanism to adaptively select a threshold $\gamma_k$  for each class based on the level of difficulty. FlexMatch has demonstrated improvement against the state-of-the-art methods, such as FixMatch \cite{sohn2020fixmatch} and MixMatch \cite{berthelot2019mixmatch}, on large-scale image classification tasks.  


\textbf{Related work using uncertainty in SSL.} Several works \cite{yu2019uncertainty,xia20203d,mukherjee2020uncertainty,shi2021inconsistency,zheng2021rectifying} have considered using uncertainty estimation to improve consistency regularization for SSL. %Recent research has also tackled SSL with uncertainty for graph data \cite{zhao2020uncertainty}.
%use uncertainty to improve consistency regularization learning for the segmentation of medical images. A concurrent work \cite{mukherjee2020uncertainty}, selects pseudo-labels predicted by a pretrained language model using uncertainty for a downstream SSL task. One difference between our works is the selection of hard samples. Whereas Mukherjee et al. select a certain amount of hard samples (i.e. those which are not confident or certain) and learn from these using positive learning, we decide to use negative learning on these samples which reduces the amount of noise seen by the network. \cite{zheng2021rectifying} show strong performance on the domain adaptive semantic segmentation task by leveraging uncertainty. 
%However, to the best of our knowledge, pseudo-labeling with uncertainty consideration has not been studied in tabular data domain although such uncertainty information can reduce the effect of inconsistent , thus poor, classification in the pseudo-labeling process. 
For pseudo-labeling specifically, Rizve et al \cite{rizve2020defense}  propose an uncertainty-aware pseudo-label selection (UPS) that aims to reduce the noise in the training process by using the uncertainty score -- together with the probability score  for making assignments:
 \begin{align}
    y_i^k = \mathbb{1} \Bigl[ p( y_i = k \mid \bx_i ) \ge \gamma \Bigr] \; \mathbb{1} \Bigl[ u\bigl( p( y_i = k \mid \bx_i) \le \gamma_u \bigr) \Bigr]
\end{align}
where $\gamma_u$ is an additional threshold on the uncertainty level and $u(p)$ is the uncertainty of a prediction $p$.
As shown in \cite{rizve2020defense}, selecting predictions with low uncertainties greatly reduces the effect of poor calibration, thus improving robustness and generalization. 

%we propose an uncertainty-aware pseudo-label selection (UPS) framework that leverages the prediction uncertainty to guide the pseudo-label selection procedure. We believe pseudo labeling has been impactful due to its simplicity, generality, and ease of implementation; to this end, our proposed framework attempts to maintain these benefits, while addressing the issue of calibration to drastically improve PL performance.





%UPS does not require modality-specific augmentations and can leverage most uncertainty estimation methods in its selection process.


%The confidence thresholding heuristic used in FixMatch \cite{sohn2020fixmatch} also induces an annealing schedule: as model predictions become more confident over the course of training, unlabeled examples are more frequently assigned labels and thus more frequently contribute to model updates. However, it is generally unclear how the confidence threshold should be set since the predictions of many classifiers may not be calibrated without additional post-processing \cite{guo2017calibration}. The use of an allocation schedule in SLA \cite{tai2021sinkhorn_sla} obviates the need to manually select a confidence threshold parameter for training.




==> 8a.discussion.tex <==
%+ When given equal budget for tuning hyperparameters, the gap in performance between using SSL and using only labeled data is smaller than typically reported.


%+ Further, a large classifier with carefully chosen regularization trained on a small labeled dataset with no unlabeled data can reach very good accuracy. This demonstrates the importance of evaluating different SSL algorithms on the same underlying model.


%+ In some settings, pre-training a classifier on a different labeled dataset and then retraining on only labeled data from the dataset of interest can outperform all SSL algorithms we studied.


% + Performance of SSL techniques can degrade drastically when the unlabeled data contains a different distribution of classes than the labeled data.


%+ Different approaches exhibit substantially different levels of sensitivity to the amount of labeled and unlabeled data.


%+ Realistically small validation sets would preclude reliable comparison of different methods, models, and hyperparameter settings.


%  Discussions: Why does the proposed model (VIME) need for tabular data?
% Image and tabular data are very different. The spatial correlations between pixels in images or the
% sequential correlations between words in text data are well-known and consistent across different
% datasets. By contrast, the correlation structure among features in tabular data is unknown and varies
% across different datasets. In other words, there is no common correlation structure in tabular data
% (unlike in image and text data). This makes the self- and semi-supervised learning in tabular data
% more challenging. Note that promising methods for image domain do not guarantee the favorable
% results on tabular domain (vice versa). Also, most augmentations and pretext tasks used in image data
% are not applicable to tabular data; because they directly utilize the spatial relationship of the image for
% augmentation (e.g., rotation) and pretext tasks (e.g., jigsaw puzzle and colorization). To transfer the
% successes of self- and semi-supervised learning from image to tabular domains, proposing applicable
% and proper pretext tasks and augmentations for tabular data (our main novelty) is critical. Note that
% better augmentations and pretext tasks can significantly improve self- and semi-supervised learning
% performances.



%\paragraph{Why does Pseudo-Labeling work?}
%The goal of any Semi-Supervised Learning algorithm is to use both the unlabeled and labeled samples to learn the underlying structure of the data. Pseudo-Labeling is able to do this by making two important assumptions:
%Continuity Assumption (Smoothness): Points that are close to each other are more likely to share a label.  In other words, small changes in input do not cause large changes in output. This assumption allows pseudo labeling to conclude that small changes in images like rotation, shearing, etc do not change the label.
%Cluster Assumption: The data tend to form discrete clusters, and points in the same cluster are more likely to share a label. This is a special case of the continuity assumption Another way to look at this is -- the decision boundary between classes lies in the low-density region (doing so helps in generalization -- similar to maximum margin classifiers like SVM).


% The initial labeled data is important -- it helps the model learn the underlying cluster structure to infer labels for the unlabeled data. As the training progresses, the learned cluster structure is improved using the unlabeled data.

%\paragraph{Limitations}

%The limits of semi-supervised machine learning Semi-supervised learning is not applicable to all supervised learning tasks. As in the case of the handwritten digits, your classes should be able to be separated through clustering techniques. Alternatively, as in S3VM, you must have enough labeled examples, and those examples must cover a fair represent the data generation process of the problem space.

%But when the problem is complicated and your labeled data are not representative of the entire distribution, semi-supervised learning will not help. For instance, if you want to classify color images of objects that look different from various angles, then semi-supervised learning might help much unless you have a good deal of labeled data (but if you already have a large volume of labeled data, then why use semi-supervised learning?). Unfortunately, many real-world applications fall in the latter category, which is why data labeling jobs wont go away any time soon.

%But semi-supervised learning still has plenty of uses in areas such as simple image classification and document classification tasks where automating the data-labeling process is possible.

%Semi-supervised learning is a brilliant technique that can come handy if you know when to use it.

==> adversarial_perspective.tex <==

\subsection{Adversarial Perspective of Sampling}
In this section, we consider selecting points who are easily changed by a distributional adversary. First, we set-up some notation: let $\theta_1,\ldots,\theta_M$ correspond to the $M$ models of ensemble. The confidence of a point $\bx \in \mathcal{X}$ to class $k$ is
\begin{align}
    L(\bx; \tilde{q}) := \sum_{j=1}^M q_j P(y = k \mid \bx, \theta_j),
\end{align}
where $\tilde{q} = \bracket{q_1,\ldots,q_M}$ are the weights of each ensemble. Typically $\tilde{q}$ is taken to be a uniform weighting and we can select high confidence points by solving:
\begin{align}
    \arg\max_{\bx \in \mathcal{D}_u} L(\bx; \tilde{q}).
\end{align}
There may be bias in certain models so we consider an adversary who will select $\tilde{q}$ in the worst possible way and select examples that are vulnerable in this scheme. More specifically, we define a ball $B(\varepsilon) := \braces{\tilde{q} : \chi^2 \bigl(\tilde{q},(1/M, \ldots, 1/M) \bigr) \leq \varepsilon}$, where $\chi^2(\tilde{p},\tilde{q}) = \sum_{j} q_j \bigl( \frac{p_j}{q_j} - 1 \bigr)^2 $ is the chi-squared divergence. The overall objective we are interested in is therefore
\begin{align}
    \arg\max_{\bx \in \mathcal{D}_u} \min_{\tilde{q} \in B(\varepsilon)} L(\bx; \tilde{q}),
\end{align}
where $\varepsilon$ corresponds to the budget of the adversary. In order to tackle this objective, we present the following Theorem.
\begin{theorem}
Let $p_{mk}:= p(y=k \mid \bx, \theta_m )$. For $\varepsilon > 0$, we have
\begin{align}
\max_{\tilde{q} \in B(\varepsilon)} L(\bx; \tilde{q}) = \frac{1}{M}\sum_{m=1}^M  p_{mk} - \sqrt{\varepsilon \sum_{m=1}^M \bracket{ \frac{1}{M} p_{mk} - p_{mk} }^2 } \label{theorem-eq:selection}.
\end{align}
\end{theorem}
Notably, the term in \eqref{theorem-eq:selection} motivates an extra quantity that we will use to select points. 

\textcolor{blue}{Our theoretical result in Theorem \ref{theorem-eq:selection} presents the equivalency of (i) the selection rule using uncertainty in previous work \cite{rizve2020defense} to (ii) the adversarial robustness selection. In addition, our novel finding shows that selecting the low variance points  }

==> check_list.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please read the checklist guidelines carefully for information on how to answer these questions.  For each question, change the default \answerTODO{} to \answerYes{}, \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf justification to your answer}, either by referencing the appropriate section of your paper or providing a brief inline description.  For example:
%\begin{itemize}
  %\item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  %\item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
 % \item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your answers.  Note that the Checklist section does not count towards the page limit.  In your paper, please delete this instructions block and only keep the Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See Section \ref{sec:method} and Section \ref{sec:experiment}}
  \item Did you describe the limitations of your work?
    \answerYes{See Section \ref{sec:ablation_study}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{See Section \ref{sec:theoretical_analysis_uncertainty_pl}}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See Section \ref{sec:experiment} and Appendix \ref{app_sec_exp_settigs}. We will release the source code in the final version.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section \ref{sec:experiment}, Appendix \ref{app_sec_exp_settigs}, Table \ref{tab:xgb_hypers}, Table \ref{table:dataset}}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{All of the results are reported using $30$ independent random seeds. See Section \ref{sec:experiment}}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{We report in Appendix Section \ref{app_sec_computational_time} that the computation of our algorithm for each pseudo-labeling iteration can take within a second which is negligible. Thus, the heavy computational resource and GPU are not required.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We property cite and provide the Github link to the original codes. See the first paragraph of Section \ref{sec:experiment} }
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


